Spectroscopy-Guided Discovery of Three-Dimensional Structures of Disordered Materials with Diffusion Models

The ability to rapidly develop materials with desired properties has a transformative impact on a broad range of emerging technologies. In this work, we introduce a new framework based on the diffusion model, a recent generative machine learning method to predict 3D structures of disordered materials from a target property. For demonstration, we apply the model to identify the atomic structures of amorphous carbons ($a$-C) as a representative material system from the target X-ray absorption near edge structure (XANES) spectra--a common experimental technique to probe atomic structures of materials. We show that conditional generation guided by XANES spectra reproduces key features of the target structures. Furthermore, we show that our model can steer the generative process to tailor atomic arrangements for a specific XANES spectrum. Finally, our generative model exhibits a remarkable scale-agnostic property, thereby enabling generation of realistic, large-scale structures through learning from a small-scale dataset (i.e., with small unit cells). Our work represents a significant stride in bridging the gap between materials characterization and atomic structure determination; in addition, it can be leveraged for materials discovery in exploring various material properties as targeted.

==> Save-10-12/introduction.tex <==
\section{Introduction} \added{Tim: Needs more domain-specific narrative and citations. Also feel free to cite your own papers here.}

% Motivate the use of ML generation model
As a central problem in materials science, inverse design of novel materials entails a methodology to propose new material structures that adhere to specified target properties. In recent years, such a task has been increasingly researched with data-driven approaches thanks to the emerging capabilities of modern machine learning models. Critically, many material systems exhibit multi-to-one mapping in the structure-property space, i.e., multiple distinct structures can result in roughly the same property. It is therefore a challenge to learn the inverse mapping even if the forward mapping is fully known. To address this caveat, one viable approach is to formulate the inverse prediction problem in a probabilistic framework, for instance with a conditional generative model, that generates or samples multiple candidate material structures conditioned on a single given property.

% Discuss diffusion model for *3D* material generation 
Among the different classes of generative models, the diffusion model \cite{Sohl-Dickstein2015-DPM, Ho2020-DDPM, Song2020-unified} is particularly well suited for generating structures involving precise three-dimensional (3D) atomic coordinates, as the diffusion formulation centers around the idea of denoising perturbed or noisy prior inputs towards realistic distributions, based on a learned score function \cite{Hyvarinen2005, Vincent2011scorematching}, which has the form of a relative distance vector for atomic coordinate data. Further, when the data space is defined in terms of relative distance vectors between atoms, the score model does not observe absolute coordinates and is therefore translation-invariant. While there have been numerous works on diffusion model for molecules \cite{hoogeboom2022equivariant, jing2022torsional, vignac2022digress, xu2022geodiff, weiss2023guided}, relatively few works focus on \textit{material} atomic structures defined in periodic cell boundaries \cite{xie2021crystal, zheng2023towards}. In this work, we apply the diffusion model to perform conditional or guided generation of disordered/amorphous structures, a family of materials relevant to various application scopes, such as disordered interfaces in batteries, ..., etc. \added{Tim: Anh, help me out here?} \textcolor{brown}{For example, previous studies have revealed the presence of nanometer-thin disordered lithium at the interfaces between lithium metal and solid electrolytes in all solid state batteries.\cite{yang2021interfacial}} More specifically, we target amorphous carbons ($a$-C) as an initial case study for our method, with \textit{X-ray absorption near edge structure} (XANES) as the conditioning/guiding property. In a similar vein, Comin and Lewis \cite{comin2019deep} trained a Wasserstein autoencoder \cite{tolstikhin2017wasserstein} to generate amorphous silicon topologies. However, such a model is limited to a fixed number of atoms. On the other hand, our diffusion model approach is scale-agnostic, allowing for generation at any arbitrary scale.

% Briefly describe methodology
Our conditional diffusion model framework follows a standard format consisted a prior score model and a forward model, the former outputs the \textit{prior/unconditional score}, which is used to gradually denoise noisy priors towards realistic samples without bias, while the latter---which predicts per-atom spectral curves in this work---provides the \textit{likelihood/conditioning score} that guides the denoising iterations towards a given target property (Fig.~\ref{fig:intro}). Note that the target property is not necessarily always achievable (i.e., not all targets are realistic). In this regard, the given spectroscopy target may be more appropriately described as a guide. Importantly, the prior score model and the forward model are decoupled and can be separately trained. Further, the use of a forward model is optional, in which case the generation is simply unconditional. Further details regarding the conditional diffusion model implementation are described in the Methods section.

% Summarize results and highilights
\added{Tim: Hyuna, you can use this paragraph to help you write the results section.}
Our generation results reflect a few key properties that make the conditional diffusion model approach practical and flexible. First, as previously mentioned, the generation process is scale-agnostic, allowing training from small-scale data and inference at arbitrary scale. This property is related to the node-centric prediction of the underlying graph neural network architecture, and the generation process amounts to shifting each atom's coordinate towards realistic topologies based on its local neighborhood environment. Second, the (unconditional) generation results are shown to closely match the training distribution, specifically in terms of Steinhardt features \cite{Steinhardt1983PRB}, radial distribution function, bond angle distribution, and per-atom GAP potential energy. Importantly, the generation does not merely replicate atomic motifs from the training data, according to the Steinhard feature distributions. Third, despite strong correlation between density and $a$-C topologies, the conditioning score from the forward model exerts a definite bias over the denoising trajectory, resulting in significant changes to the generated topologies with predicted XANES spectra matching or approaching the target spectrum. Fourth, we also demonstrate the conditioning effect with an additional example, where a prior model trained with diamond and amorphous structures of the same density can be conditioned to generate amorphous topologies rather than the crystalline diamond. Lastly, we briefly analyze the effect of a tuning parameter that controls the degree of the conditioning effect over the denoising process, demonstrating that the conditional generation can be made to be ``lax''. This flexibility allows the model to potentially generate more diverse and novel structures with a less strict guiding effect.

% Caveats and future prospect
Although our present study focuses on single-element amorphous carbons conditioned by XANES spectroscopy, the conditional diffusion model framework can be extended to more general scenarios. For instance, the scale-agnostic property allows for a single large-scale (millions of atoms or more) generation learned from multiple (diverse) small-scale data. Such a ``stitching'' application is relevant to material transport simulations, where a large length scale is required for collecting significant and diverse transport statistics. Second, the framework can be naturally extended to multi-element material systems, where the atom type information is also subject to noising/denoising. Multi-element, disordered systems are critical to ... \added{Tim: Anh, help me out?} \textcolor{brown}{This expansion is particularly critical in addressing the intricacies of multi-element, disordered systems, crucial for generating polymers with specific target properties, such as thermal conductivity\cite{ma2022exploring} or phosphorescence\cite{guo2022long,li2022stimulus}.} Lastly, multi-target inverse prediction is also straightforward to implement, as the conditional/posterior score function is a simple summation of the prior score with the likelihood scores from multiple forward models (further details in Methods). This setup enables robust material inverse design for various target properties. Part of our future work will focus on the aforementioned applications, as well as implementation optimization for faster sampling.


\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/intro.pdf}
    \caption{The conditional generative/denoising process of amorphous carbon ($a$-C) involves a pair of decoupled (i.e., trained separately) score model and forward model. The score model, based on the diffusion model formalism, provides the prior score, while the forward model, trained to predict spectroscopic curves, is used to provide the likelihood score. The prior score serves to denoise initial random motifs towards realistic topologies without bias, and the likelihood score serves to bias the denoising trajectory towards atomic motifs that satisfy a given spectroscopic target/guide. Notably, the forward model is optional, and the generative process is simply unconditional without a forward model.
    }
    \label{fig:intro}
\end{figure}





% Spectroscopy methods, notably X-ray absorption near edge structure (XANES), are powerful tools for characterizing materials and molecular systems, providing valuable atomic structural insights. Although already highly useful, these methods may be further supplemented with models capable to proposing precise atomic structures that comply with given spectroscopic signatures. Such a capability not only serves to complement the structural information provided by spectroscopy, but also in the broader context establishes a connection to a central challenge in materials science: the task of inverse prediction of a material's precise structure based on a target or observed property.

% In the case of amorphous carbon ($a$-C), a particularly complex material, the density and XANES spectra are strongly correlated, making it difficult to deduce the precise three-dimensional atomistic structure solely from XANES data \cite{gago2000bonding}. Furthermore, the global XANES spectroscopy, which represents the average of local XANES spectra of all atoms in the system, does not exhibit a straightforward one-to-one correspondence with the atomic structure of the material. These inherent complexities make the problem particularly daunting. In this work, we developed and applied a general inverse prediction framework (i.e., applicable to non-spectroscopy data) to the XANES spectra of $a$-C systems, with clear demonstration that the inverse-predicted structures are influenced by spectroscopic input.

% This paper extends the integration of AI and machine learning in materials science, building on the foundational work of Sridharan et al.\cite{sridharan2022deep} and Carbone et al.\cite{carbone2019classification} While machine learning has shown promise in reverse engineering molecular structures from complex spectroscopic data and probing local chemical environments, the accurate extraction of three-dimensional atomic coordinates from XANES spectra remains an open challenge. To our knowledge, no existing approach has successfully addressed the task of generating precise atomic structures from spectroscopic data.

% Furthermore, our work is inspired by the innovative Crystal Diffusion Variational Autoencoder (CDVAE) introduced by Xie et al.\cite{xie2021crystal}. CDVAE presents a transformative approach to generating periodic structures of stable materials, addressing the intricate challenges imposed by quantum mechanics and atom bonding preferences. This model serves as a pivotal reference for our research, advancing the state of material generation through a physically grounded framework.

% In the broader context of generative models, several noteworthy developments have emerged.  Long et al.\cite{long2021constrained} introduce a generative model that optimizes the formation energy of crystal structures efficiently, transforming materials discovery. Notably, the research by Fung et al. has introduced invertible neural networks\cite{fung2021inverse, fung2022atomic} for materials design. Additionally, the E(3) Equivariant Diffusion Model (EDM) by Hoogeboom and Satorras\cite{hoogeboom2022equivariant} and 'TSDiff' by Kim et al.\cite{kim20232d} have demonstrated the utility of diffusion-based approaches in predicting molecular structures and transition state geometries. Turning to amorphous systems, Comin and Lewis \cite{comin2019deep} introduce a deep learning approach for modeling the atomic structure of amorphous silicon, a step forward in generating state-of-the-art structures. Kilgour et al.\cite{kilgour2020generating} pioneer a method based on deep learning to autonomously generate disordered molecular aggregates, bridging the gap between nanoscale and mesoscale simulations.

% Accurately determining atomic coordinates within amorphous or disordered systems is critical for understanding their properties. Despite its significance, reconstructing three-dimensional Cartesian atomic positions from XANES spectra remains a challenging task, receiving limited attention to date.This paper addresses this critical gap by introducing an innovative approach that unifies XANES spectroscopy with advanced generative AI models. Specifically designed for reconstructing atomic positions within amorphous structures, our framework accommodates multiple possible structures corresponding to the XANES spectra, acknowledging the inherent probabilistic nature of the problem.

% Our framework, a conditional diffusion model, probabilistically generates atomic structures based on given spectroscopy curves. This approach naturally extends the diffusion model to conditional generation, flexibly incorporating various forward models for different property conditions.(Figure\ref{fig:intro})

% First, thanks to the underlying graph neural network architecture, which yields node-centric predictions, the generation is \textit{scale-agnostic}. In other words, the denoising process amounts to shifting each atom's location towards realistic topologies based on its local environment, without regard to global variables. This also means that our model can learn from small-scale MD trajectories (e.g., hundreds of atoms) and generate structures at a larger scale (e.g., thousands of atoms or more). Second, the generated structures are realistic both geometrically and energetically, based on several geometric descriptions and energy calculations from the GAP interatomic potential. Third, spectroscopic targets clearly impact generation outcomes. For example, the generation can be steered, with provided spectroscopic inputs, to result in higher portions of \textit{sp}- or \textit{sp3}-carbons in \textit{sp2}-dominant structures. In another example, the generation is guided by spectroscopy to result in amorphous structures from a manually biased starting point that would otherwise lead to crystalline diamond topology by default.

% The significance of this research extends to advancing structural inferences derived from spectroscopy and broadening the scope of existing generative model-based inverse prediction methods to encompass amorphous and disordered structures within periodic cells. Also, the methodologies introduced in this research hold the potential for broad application beyond XANES spectroscopy and amorphous carbon systems. The flexibility of the framework can be extended to various spectroscopic techniques such as X-ray photoelectron spectroscopy (XPS), enabling the inference of atomic structures from a broader range of experimental data.
